Least costly energy management for series hybrid electric vehicles

Energy management of plug-in Hybrid Electric Vehicles (HEVs) has different challenges from non-plug-in HEVs, due to bigger batteries and grid recharging. Instead of tackling it to pursue energetic efficiency, an approach minimizing the driving cost incurred by the user - the combined costs of fuel, grid energy and battery degradation - is here proposed. A real-time approximation of the resulting optimal policy is then provided, as well as some analytic insight into its dependence on the system parameters. The advantages of the proposed formulation and the effectiveness of the real-time strategy are shown by means of a thorough simulation campaign.

==> ftp75_tcms_cost2go.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{013}[bc][bc]{\matlabtextA $J_k(x(k))$ (\euro)}%
\psfrag{014}[bc][bc]{\matlabtextA $q_b (\%)$}%
\psfrag{015}[tc][tc]{\matlabtextA time (s)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[cb][cb]{\matlabtextA $0$}%
\psfrag{001}[cb][cb]{\matlabtextA $0.1$}%
\psfrag{002}[cb][cb]{\matlabtextA $0.2$}%
\psfrag{003}[cb][cb]{\matlabtextA $0.3$}%
\psfrag{004}[cb][cb]{\matlabtextA $0.4$}%
\psfrag{005}[cb][cb]{\matlabtextA $0.5$}%
\psfrag{006}[ct][ct]{\matlabtextA $0$}%
\psfrag{007}[ct][ct]{\matlabtextA $500$}%
\psfrag{008}[ct][ct]{\matlabtextA $1000$}%
\psfrag{009}[ct][ct]{\matlabtextA $1500$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextA $48$}%
\psfrag{011}[rc][rc]{\matlabtextA $50$}%
\psfrag{012}[rc][rc]{\matlabtextA $52$}%
%
%% </ytick>

==> ftp75_tcms_sensitivity_dp.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[tc][tc]{\matlabtextA $\gamma$ (\euro/kWh)}%
\psfrag{011}[bc][bc]{\matlabtextA $p(0)-p(T)$ (-)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0.05$}%
\psfrag{001}[ct][ct]{\matlabtextA $0.1$}%
\psfrag{002}[ct][ct]{\matlabtextA $0.15$}%
\psfrag{003}[ct][ct]{\matlabtextA $0.2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextA $-0.1$}%
\psfrag{005}[rc][rc]{\matlabtextA $0$}%
\psfrag{006}[rc][rc]{\matlabtextA $0.1$}%
\psfrag{007}[rc][rc]{\matlabtextA $0.2$}%
\psfrag{008}[rc][rc]{\matlabtextA $0.3$}%
\psfrag{009}[rc][rc]{\matlabtextA $0.4$}%
%
%% </ytick>

==> ftp75_tcms_sensitivity_dx.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[tc][tc]{\matlabtextA $\gamma$ (\euro/kWh)}%
\psfrag{011}[bc][bc]{\matlabtextA $q_b(0)-q_b(T)$ (\%)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0.05$}%
\psfrag{001}[ct][ct]{\matlabtextA $0.1$}%
\psfrag{002}[ct][ct]{\matlabtextA $0.15$}%
\psfrag{003}[ct][ct]{\matlabtextA $0.2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextA $-4$}%
\psfrag{005}[rc][rc]{\matlabtextA $-2$}%
\psfrag{006}[rc][rc]{\matlabtextA $0$}%
\psfrag{007}[rc][rc]{\matlabtextA $2$}%
\psfrag{008}[rc][rc]{\matlabtextA $4$}%
\psfrag{009}[rc][rc]{\matlabtextA $6$}%
%
%% </ytick>

==> ftpMix_tcms_sensitivity_dp.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[tc][tc]{\matlabtextA $\gamma$ (\euro/kWh)}%
\psfrag{011}[bc][bc]{\matlabtextA $p(0)-p(T)$ (-)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0.05$}%
\psfrag{001}[ct][ct]{\matlabtextA $0.1$}%
\psfrag{002}[ct][ct]{\matlabtextA $0.15$}%
\psfrag{003}[ct][ct]{\matlabtextA $0.2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextA $-1$}%
\psfrag{005}[rc][rc]{\matlabtextA $-0.5$}%
\psfrag{006}[rc][rc]{\matlabtextA $0$}%
\psfrag{007}[rc][rc]{\matlabtextA $0.5$}%
\psfrag{008}[rc][rc]{\matlabtextA $1$}%
\psfrag{009}[rc][rc]{\matlabtextA $1.5$}%
%
%% </ytick>

==> ftpMix_tcms_sensitivity_dx.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{009}[tc][tc]{\matlabtextA $\gamma$ (\euro/kWh)}%
\psfrag{010}[bc][bc]{\matlabtextA $q_b(0)-q_b(T)$ (\%)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0.05$}%
\psfrag{001}[ct][ct]{\matlabtextB $0.1$}%
\psfrag{002}[ct][ct]{\matlabtextB $0.15$}%
\psfrag{003}[ct][ct]{\matlabtextB $0.2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextB $-10$}%
\psfrag{005}[rc][rc]{\matlabtextB $0$}%
\psfrag{006}[rc][rc]{\matlabtextB $10$}%
\psfrag{007}[rc][rc]{\matlabtextB $20$}%
\psfrag{008}[rc][rc]{\matlabtextB $30$}%
%
%% </ytick>
